Learning A Physical Long-term Predictor

Evolution has resulted in highly developed abilities in many natural intelligences to quickly and accurately predict mechanical phenomena. Humans have successfully developed laws of physics to abstract and model such mechanical phenomena. In the context of artificial intelligence, a recent line of work has focused on estimating physical parameters based on sensory data and use them in physical simulators to make long-term predictions. In contrast, we investigate the effectiveness of a single neural network for end-to-end long-term prediction of mechanical phenomena. Based on extensive evaluation, we demonstrate that such networks can outperform alternate approaches having even access to ground-truth physical simulators, especially when some physical parameters are unobserved or not known a-priori. Further, our network outputs a distribution of outcomes to capture the inherent uncertainty in the data. Our approach demonstrates for the first time the possibility of making actionable long-term predictions from sensor data without requiring to explicitly model the underlying physical laws.

==> 05b_longTermPrediction_figure.tex <==
\iftrue
\begin{figure*}[t]
    \vspace{-0.1in}
    \centering\resizebox{0.9\textwidth}{!}{
    \begin{overpic}[width=\linewidth]{images/result_graphs/graph_all}
    %\includegraphics[width=\linewidth]{images/result_graphs/graph_all.pdf}
    \put(18,-0.1){(a)}
    \put(50.5,-0.1){(b)}
    \put(83,-0.1){(c)}
    \end{overpic}
    }
    \vspace{-0.1in}
    \caption{\textbf{Long term prediction evolutions}. Comparison of network trained using sequences of length 20. Error bars denote $25^{th}$ and $75^{th}$ percentiles of the $L^2$ loss in pixels.}\label{fig:result_graphs}
        
    % The baselines (Linear and Quadratic) were fit to the first 10 frames, all other networks had to make predictions after having seen the first $\ninputs=4$ frames. Note, how deterministic predictors cannot handle situations with unforeseen circumstances (\textit{i.e.}, heterogeneous friction of the slope). The training set consisted of 8750 scenes. Error bars denote $25^{th}$ and $75^{th}$ percentiles of the $L^2$ loss in pixels (the image size was $128\times128$) evaluated over 3750 test cases.

    %\vspace{-0.2in}
\end{figure*}
\else
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/result_graphs/graph_S0}
    \caption{
    Comparison of long-term prediction accuracy of baselines and proposed networks in the least complex scenario \szero.
    %Comparison of prediction accuracy of baseline predictors using $\ninputs$ images as input, and predicting $16,~23,~26, \ldots$ timesteps ahead. Units (pixels?). Mark $\ninputs$. Log plot?
    }
    \label{fig:result_s0}
\end{figure}

==> 07_scratch.tex <==
\clearpage\section*{Scratch}

\input{results_plate}
\input{results_pdfs}
\input{results_trainmore}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/result_graphs/graph_S1}
    \caption{Comparison of long-term prediction accuracy of baselines and proposed networks in the varying plane rotation scenario \sone.}
    \label{fig:result_s1}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/result_graphs/graph_S2}
    \caption{Comparison of long-term prediction accuracy of baselines and proposed networks in the varying plane rotation scenario \stwo.}
    \label{fig:result_s2}
\end{figure}
\fi

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/result_graphs/graph_entropy}
    \caption{Shannon entropy evolution of \NetThree\ and \NetFour\ on Scenario~\sone. \NetThree entropy  is the continuous extension of Shannon discrete entropy. Error bars denote $25^{th}$ and $75^{th}$ percentiles of the Shannon entropy}
    \label{fig:entropy}
\end{figure}


==> results_trainmore.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_02_time_40_heatmap_20.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_02_time_40_heatmap_30.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_02_time_40_heatmap_40.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_03_time_40_heatmap_20.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_03_time_40_heatmap_30.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_03_time_40_heatmap_40.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_06_time_40_heatmap_20.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_06_time_40_heatmap_30.pdf}
\includegraphics[width=0.32\linewidth]{images/results/S1_samples/S1_06_time_40_heatmap_40.pdf}
\caption{The effect of training \NetFour for longer times (columns: 20, 30, 40) in Scenario S1.}
\label{fig:results_trainmore_S1}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_02_time_all_heatmap_20.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_02_time_all_heatmap_30.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_02_time_all_heatmap_40.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t=[20, 30, 40]$) in Scenario S1, column 1 in \cref{fig:results_allcomp_S1}.}
\label{fig:results_softmax_over_time_S1_1}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_03_time_all_heatmap_20.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_03_time_all_heatmap_30.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_03_time_all_heatmap_40.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t=[20, 30, 40]$) in Scenario S1, column 2 in \cref{fig:results_allcomp_S1}.}
\label{fig:results_softmax_over_time_S1_2}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_06_time_all_heatmap_20.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_06_time_all_heatmap_30.pdf}
\includegraphics[width=1.00\linewidth]{images/results/S1_samples/S1_06_time_all_heatmap_40.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t=[20, 30, 40]$) in Scenario S1, column 3 in \cref{fig:results_allcomp_S1}.}
\label{fig:results_softmax_over_time_S1_3}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S2_samples/S2_04_time_all_heatmap_30.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t= 30$) in Scenario S2, column 1 in \cref{fig:results_allcomp_S2}.}
\label{fig:results_softmax_over_time_S2_1}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S2_samples/S2_05_time_all_heatmap_30.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t=30$) in Scenario S2, column 2 in \cref{fig:results_allcomp_S2}.}
\label{fig:results_softmax_over_time_S2_2}\end{figure*}
\begin{figure*}[h]
\centering
\includegraphics[width=1.00\linewidth]{images/results/S2_samples/S2_07_time_all_heatmap_30.pdf}
\caption{Evolution of predictions for different versions of \NetFour(rows: trained for $t=30$) in Scenario S2, column 3 in \cref{fig:results_allcomp_S2}.}
\label{fig:results_softmax_over_time_S2_3}\end{figure*}

